Provably Efficient Cooperative Multi-Agent Reinforcement Learning with Function Approximation

Reinforcement learning in cooperative multi-agent settings has recently advanced significantly in its scope, with applications in cooperative estimation for advertising, dynamic treatment regimes, distributed control, and federated learning. In this paper, we discuss the problem of cooperative multi-agent RL with function approximation, where a group of agents communicates with each other to jointly solve an episodic MDP. We demonstrate that via careful message-passing and cooperative value iteration, it is possible to achieve near-optimal no-regret learning even with a fixed constant communication budget. Next, we demonstrate that even in heterogeneous cooperative settings, it is possible to achieve Pareto-optimal no-regret learning with limited communication. Our work generalizes several ideas from the multi-agent contextual and multi-armed bandit literature to MDPs and reinforcement learning.

==> bak.tex <==
Reinforcement learning in cooperative multi-agent settings has recently advanced significantly in its scope, with applications in cooperative estimation for advertising, dynamic treatment regimes, distributed control, and federated learning. In this talk, we will discuss the problem of cooperative multi-agent RL with function approximation, where a group of agents communicates with each other to jointly solve an episodic MDP lying in a known function class. We propose efficient algorithms for two communication protocols - (i) centralized learning, where the agents communicate via a centralized server, and (ii) decentralized learning, where agents communicate via peer-to-peer messages on a network with delays. Our key contributions are as follows. First, in both centralized and decentralized fully-cooperative settings, we demonstrate that via careful message-passing and cooperative value iteration, it is possible to achieve near-optimal no-regret learning even with a fixed constant communication budget. Next, we demonstrate that even in heterogeneous cooperative settings, it is possible to achieve Pareto-optimal no-regret learning with limited communication. Our work generalizes several ideas from the multi-agent contextual bandit literature to MDPs and leverages techniques from vector-valued statistical learning theory.

Reinforcement learning in cooperative multi-agent settings has recently advanced significantly in its scope, with applications in cooperative estimation for advertising, dynamic treatment regimes, distributed control, and federated learning. In this paper, we discuss the problem of cooperative multi-agent RL with function approximation, where a group of agents communicates with each other to jointly solve an episodic MDP. Our key contributions are as follows. We demonstrate that via careful message-passing and cooperative value iteration, it is possible to achieve near-optimal no-regret learning even with a fixed constant communication budget. Next, we demonstrate that even in heterogeneous cooperative settings, it is possible to achieve Pareto-optimal no-regret learning with limited communication. Our work generalizes several ideas from the multi-agent contextual bandit literature to MDPs and leverages techniques from vector-valued statistical learning.

==> main_paper.tex <==

\section{Introduction}
Cooperative multi-agent reinforcement learning systems are widely prevalent in several engineering applications, e.g., robotic systems~\citep{ding2020distributed}, power grids~\citep{yu2014multi}, traffic control~\citep{bazzan2009opportunities}, as well as team games~\citep{zhao2019multi}. Increasingly, federated~\citep{yang2019federated} and distributed~\citep{peteiro2013survey} machine learning is gaining prominence in industrial applications, and reinforcement learning in these large-scale settings is becoming of import in the research community as well~\citep{zhuo2019federated, liu2019lifelong}. Additionally, recent research in the statistical machine learning community has focused on designing cooperative multi-agent decision-making algorithms with provable performance  guarantees~\citep{zhang2018fully, wai2018multi, zhang2018networked}. 

In this paper, we study cooperative multi-agent reinforcement learning in the context of two practical scenarios - the first, which we denote \textit{independent} multi-agent MDPs, corresponds to the federated and distributed RL setting, where a group of agents simultaneously solve their own independent MDPs that are assumed to be ``similar'' to each other, and communicate to facilitate faster learning. The second is the (cooperative) simultaneous-move Markov game setting, where a group of agents interact with the same MDP with simultaneous moves, and the objective is to recover Pareto-optimal multi-agent policies. The latter environment corresponds to general cooperative Markov games, such as multi-agent robotics.

For each of these settings, our objective is to design algorithms that recover the optimal \textit{centralized} performance guarantees, while at the same time limiting the amount of communication between agents.

\section{Background and Preliminaries}
\textbf{Notation}. We denote vectors by lowercase solid characters, i.e., $\x$ and matrices by uppercase solid characters $\bX$, and sets by calligraphic characters, i.e., $\cX$. We denote the $\bS-$ellipsoid norm of a vector $\x$ as $\lVert \x \rVert_\bS = \sqrt{\x^\top\bS\x}$. That a symmetric matrix $\bA$ is positive semi-definite (PSD) is given by $\bA \succcurlyeq {\bf 0}$, and the L\"owner ordering of symmetric PSD matrices by $\bA \succcurlyeq \bB$, which implies $\bA - \bB \succcurlyeq {\bf 0}$. The indicator function is given by $\bone$, and the probability of an event $A$ is given by $\bbP(A)$. We denote the interval $a, a+1, ..., b$ for $b \geq a$ by $[a, b]$ and simply by $[b]$ when $a=1$.

\subsection{Multi-Agent Markov Decision Processes}
We focus only on episodic Markov Decision Processes (MDPs) in the multi-agent setting. We consider two variants of multi-agent environments - (i) independent, where the environments for each agent are independent of each other, e.g., in the federated reinforcement learning setting, and (ii) the traditional Markov game setting.

\subsubsection{Federated Multi-Agent MDPs}

In the \textit{federated} setting, each agent $m \in [M]$ interacts with a (possibly unique) isolated episodic MDP, with a common action space and state space, but possibly unique reward functions and transition probabilities. This does not imply that the agents \textit{share} a state space as in the Markov game setting, but that their MDPs are isolated but only share common state and action spaces. An example of such a setting would be two different games on an Atari console - while the state space for each of the two games potentially is all possible pixel arrangements of the console, and action space is given by the (common) set of controls, these are independent, episodic MDPs. 

Formally, the MDP for agent $m \in [M]$ is given by $\text{MDP}(\cS, \cA, H, \bbP_m, \br_m)$, where the state and action spaces are given by $\cS$ and $\cA$ respectively, the reward functions $\br_m = \{r_{m, h}\}_{h \in [H]}, r_{m, h} : \cS \times \cA \rightarrow [0, 1]$\footnote{We consider $r_{m, h}$ to be deterministic and bounded for simplicity, however, our results can trivially be extended to random sub-Gaussian rewards as well.}, and transition probabilities $\bbP_m = \left\{\bbP_{m, h}\right\}_{h \in [H]} , \bbP_{m, h} : \cS \times \cA \rightarrow \cS$, i.e., $\bbP_{m, h}(x' | x, a)$ denotes the probability of the agent moving to state $x'$ if at step $h$ it selects action $a$ from state $x$. We assume that $\cS$ is measurable with possibly infinite elements, and that $\cA$ is finite with some size $A$. For any agent $m$, the policy $\pi_m$ is a set of $H$ functions $\pi_m = \{\pi_{m, h}\}_{m \in [M]}, \pi_{m, h} : \cS \rightarrow \cA$ such that $\sum_{a \in \cA} \pi_{m, h}(a|x) = 1 \ \forall \ x \in \cS$ and $\pi_{m, h}(a|x)$ is the probability of agent $m$ taking action $a$ from state $x$ at step $h$.

In the independent setting, the problem proceeds as follows. At every episode $t \in [T]$, each agent $m \in [M]$ starts out with a policy $\pi^t_m = \{\pi^t_{m, h}\}_{h \in [H]}$ in an initial state $x^t_{m, 1}$ picked arbitrarily by the environment. For each step $h \in [H]$ of the episode, each agent observes its state $x^t_{m, h}$, selects an action $a^t_{m, h} \sim \pi^t_{m, h}(\cdot | x^t_{m, h})$, obtains a reward $r_{m, h}(x^t_{m, h}, a^t_{m, h})$, and transitions to state $x^t_{m, h+1}$ sampled according to $\bbP_{m, h}(\cdot | x^t_{m, h}, a^t_{m, h})$. The episode terminates at step $H+1$ where all agents receives zero reward. After termination, the agents can communicate among themselves via a centralized protocol (i.e., with a server), or decentralized message passing over a network. The performance of any policy $\pi$ in the $m^{th}$ MDP is measured by the value function $V^\pi_{m, h}(x) : \cS \rightarrow \bbR$, defined for all $x \in \cS, h \in [H], m \in [M]$ as,
\begin{align*}
    V^\pi_{m, h}(x) := \bbE_\pi\left[ \sum_{i=h}^{H} r_{m, i}(x_i, a_i) \ \Big| \ x_h = x\right].
\end{align*}
The expectation is taken with respect to the random trajectory followed by the agent in the $m^{th}$ MDP. A related function $Q^\pi_{m, h} : \cS \times \cA \rightarrow \bbR$ determines the total expected reward from any action-state pair at step $h$ for the $m^{th}$ MDP for any state $x \in \cS$ and action $a \in \cA$:
\begin{align*}
    Q^\pi_{m, h}(x, a) := \bbE_\pi\left[ \sum_{i=h}^{H} r_{m, i}(x_i, a_i) \ \Big| \ (x_h, a_h) = (x, a)\right]. 
\end{align*}
Let $\pi^\star_m$ denote the optimal policy for the $m^{th}$ MDP, i.e., the policy that gives the maximum value, $V^\star_{m, h}(x) = \sup_{\pi}V^\pi_{m, h}(x)$, for all $x \in \cS, h \in [H]$. Each MDP has its own unique optimal policy $\pi^\star_{m, h}$. For $T$ episodes, the cumulative regret (in expectation), is defined as,
\begin{align*}
    \regret(T) := \sum_{m=1}^M \sum_{t=1}^T \left[V^\star_{m, 1}(x^t_{m, 1}) -  V^{\pi_{m, t}}_{m, 1}(x^t_{m, 1})\right].
\end{align*}
\textbf{Homogeneous Environments}. The \textit{homogeneous} environment is a special case of the above problem, when each agent interacts with the same MDP. In this case, $\br_1 = \br_2 = \dots = \br_M = \br$ and $\bbP_1 = \bbP_2 = \dots = \bbP_M = \bbP$. Moreover, we have that the optimal policy for all agents is identical as well. This setting is common in applications such as federated learning. We treat the homogenous case separately with a simpler algorithm, and refer to the general case as the \textit{heterogeneous} independent setting.

\subsubsection{Episodic Markov Games}

The alternative setting we consider is the episodic Markov game, which can be seen as an extension of an MDP to multiple agents~\citep{}. The Markov game can be formally described as $\text{MG}(\cS, \cM, \cA, H, \bbP, \bR)$, where the set of agents $\cM$ is finite and countable with cardinality $M$, the state and action spaces are factorized as $\cS = \cS_1 \times \cS_2 \times \dots \cS_M$ and $\cA = \cA_1 \times \cA_2 \times \dots \cA_M$, where $\cS_i$ and $\cA_i$ denote the individual state and action space for agent $i$ respectively. Furthermore, the transition matrix $\bbP = \{\bbP_h\}_{h \in [H]}$ depends on the joint action-state configuration for all agents, i.e., $\bbP_h : \cS \times \cA \rightarrow \cS$, and so does the (vector-valued) reward function $\bR = \{\br_h\}_{h \in [H]}, \br_h : \cS \times \cA \rightarrow \bbR^M$.

The Markov game proceeds as follows. In each episode $t \in [T]$ each agent fixes a policy $\pi^t_m = \{\pi^t_{m, h}\}_{h \in [H]}$ in a common initial state $\x^t_{1} = \{x^t_{m, 1}\}_{h \in [H]}$ picked arbitrarily by the environment. For each step $h \in [H]$ of the episode, each agent observes the overall state $\x^t_{h}$, selects an individual action $a^t_{m, h} \sim \pi^t_{m, h}(\cdot | \x^t_{h})$ (denoted collectively as the joint action $\ba^t_h = \{a^t_{m, h}\}_{m \in \cM}$), and obtains a reward $r_{m, h}(\x^t_{h}, \ba^t_{h})$ (denoted collectively as the joint reward $\br_h(\x^t_{h}, \ba^t_{h}) = \{r_{m, h}(\x^t_{h}, \ba^t_{h})\}_{m \in \cM}$). All agents transition subsequently to a new joint state $\x^t_{h+1} = \{x^t_{m, h+1}\}_{m \in \cM}$ sampled according to $\bbP_{h}(\cdot | \x^t_{h}, \ba^t_{h})$. The episode terminates at step $H+1$ where all agents receive zero reward. After termination, the agents can communicate among themselves via a centralized protocol (i.e., with a server), or decentralized message passing over a network. 

Let $\bpi = \{\bpi_h\}_{h \in [H]}, \bpi_h = \{\pi_{m, h}\}_{m \in \cM}$ denote the joint policy for all $M$ agents. We can define the vector-valued value function over all states $\x \in \cS$ for a policy $\bpi$ as,
\begin{align*}
    \bV^\bpi_h(\x) := \bbE_\bpi\left[ \sum_{i=h}^H \br_i(\x_i, \ba_i) \ \Big| \ \x_h = \x \right].
\end{align*}
Additionally, one can define the analogous vector-valued Q-function for a policy $\bpi$ and any $\x \in \cS, \ba \in \cA, h \in [H]$,
\begin{align*}
    &\bQ^\bpi_h(\x, \ba) :=\\ &\br_h(\x, \ba) + \bbE_\bpi\left[ \sum_{i=h+1}^H \br_i(\x_i, \ba_i) \ \Big| \ (\x_h, \ba_h) = (\x, \ba) \right].
\end{align*}

Without restrictions, a general Markov game represents a wide variety of environments, including competitive zero-sum settings as well as cooperative settings. We focus on recovering the set of \textit{cooperative} Pareto-optimal policies, i.e., policies that cannot improve any individual agent's cumulative reward without decreasing the reward of the other agents. Specifically, a (multi-agent) policy $\bpi$ Pareto-dominates another policy $\bpi'$ iff $\bV^\bpi_1(\x) \succeq \bV^{\bpi'}_1(\x) \forall \ \x \in \cS$. Consequently, a policy is Pareto-optimal if it is not Pareto-dominated by any other policy. Let us denote the set of all possible multi-agent policies by $\bPi$, and the set of Pareto-optimal policies by $\bPi^\star$. Our goal is to recover the set of Pareto-optimal policies $\bPi^\star$ with high probability. 


As is commonly done in multi-objective optimization, our approach would be to utilize the method of \textit{scalarization}, where we define a (user-defined) probability distribution over the Pareto-optimal policies by converting the vector-valued Value function to a parameterized scalar measure. Consider a \textit{scalarization function} $\fs_\bupsilon(\x) = \bupsilon^\top\x : \bbR^M \rightarrow \bbR$ parameterized by $\bupsilon$ belonging to  $\bUpsilon \subseteq \Delta^M$. We then have the \textit{scalarized value function} $V^\bpi_{\bupsilon, h}(x) : \cS \rightarrow \bbR$, defined for some joint policy $\bpi$ as,
\begin{align}
    V^\bpi_{\bupsilon, h}(\x) := \fs_\bupsilon(\bV^\bpi_h(\x)) = \fs_\bupsilon\bV^\bpi_h(\x).
    \label{eqn:v_scalarized}
\end{align}
The related function $Q^\bpi_{\bupsilon, h} : \cS \times \cA \rightarrow \bbR$ is defined as,
\begin{align}
    Q^\bpi_{\bupsilon, h}(\x, \ba) := \fs_\bupsilon(\bQ^\bpi_h(\x, \ba)) = \fs_\bupsilon\bQ^\bpi_h(\x, \ba).
    \label{eqn:q_scalarized}
\end{align}
Since both $\cA$ and $H$ are finite, there exists an optimal policy for a fixed scalarization $\bupsilon$, which gives the optimal value $V^\star_{\bupsilon, h} = \sup_{\bpi \in \bPi} V^\bpi_{\bupsilon, h}(\x)$ for all $\x \in \cS$ and $h \in [H]$.
\begin{proposition}
\label{prop:mg_bellman_optimal}
For the scalarized value function given in Equation~\ref{eqn:v_scalarized}, the Bellman optimality equations are given as, for all $h \in [H], \x \in \cS, \ba \in \cA, \bupsilon \in \bUpsilon$,
\begin{align*}
    Q^\star_{\bupsilon, h}(\x, \ba) &= \fs_\bupsilon\br_h(\x, \ba) + \bbP_h V^\star_{\bupsilon, h}(\x, \ba),\\
    V^\star_{\bupsilon, h}(\x) &= \max_{\ba \in \cA} Q^\star_{\bupsilon, h}(\x, \ba)\text{ and},\\
    V^\star_{\bupsilon, H+1}(\x) &= 0.
\end{align*}
\end{proposition}
It is evident that the optimal policy for any fixed $\bupsilon$ is given by the greedy policy with respect to the Bellman-optimal scalarized Q values. We denote this (unique) optimal policy by $\pi^\star_{\bupsilon}$. We now demonstrate that each policy $\bpi^\star_\bupsilon$ lies in the Pareto frontier.
\begin{proposition}
For any fixed scalarization parameter $\bupsilon \in \bUpsilon$, the optimal greedy policy $\bpi^\star_\bupsilon$ with respect to the scalarized Q-value that satisfies Proposition~\ref{prop:mg_bellman_optimal} lies within the Pareto frontier $\bPi^\star$.
\end{proposition}
In this paper, we consider a Bayesian approach (inspired by multi-objective optimization~\citep{}) and assume a prior distribution $p_\bUpsilon(\cdot)$ over the scalarization weight with support $\bUpsilon$. We will minimize the Bayes regret over $\bUpsilon$, given by,
\begin{align}
    \regret_\bUpsilon(T) := \bbE_{\bupsilon \sim p_\bUpsilon}\left[ \sum_{t=1}^T \left[V^\star_{\bupsilon, 1}(\x^t_{1}) -  V^{\pi_{\bupsilon, t}}_{\bupsilon, 1}(\x^t_{1})\right]\right].
\end{align}

\section{Algorithm for Independent MDPs}
Here, we introduce the algorithm for independent MDPs. Our algorithms are a variant of least-squares value iteration with optimism~\citep{yang2020provably}. The motivation behind algorithm design in this setting is to strategically allow for communication between the agents such that with minimal overhead, we achieve a regret close to the single-agent case. The central idea behind value iteration is to obtain the optimal Q-values $\{Q^\star_{m, h}\}_{h \in [H], m \in \cM}$ by recursively applying the Bellman equation. Specifically, each agent $m \in [M]$ constructs a sequence of action-value functions $\{Q_{m, h}\}_{h \in [H]}$ as, for each $x \in \cS, a \in \cA, h \in [M]$,
\begin{equation*}
Q_{m, h}(x, a) \leftarrow \bbT^\star_{m, h} Q_{m ,h+1} = \left[r_{m, h} + \bbP_hV_{m, h+1}\right](x, a),
\end{equation*}
\begin{equation*}
V_{m, h+1}(x, a) \leftarrow \max_{a' \in \cA} Q_{m, h+1}(x, a').
\end{equation*}
Our approach in the general function approximation setting is to solve a least-squares regression problem based on \textit{multi-agent} historical data. For a function class $\cF$, assume that any agent $m \in [M]$ has observed $t_m$ transition tuples $\{x^\tau_h, a^\tau_h, x^\tau_{h+1}\}_{\tau \in [t_m]}$ for any step $h \in [H]$. Then, the agent estimates the optimal Q-value for any step by LSVI, by solving the regularized least-squares regression:
\begin{align*}
\widehat Q^t_{m, h} \leftarrow \argmin_{f \in \cF}\left\{\sum_{\tau \in [t_m]} \left[y^\tau_h - f(x^\tau_h, a^\tau_h)\right]^2 + \lVert f \rVert\right\}.
\end{align*}
Here, the targets $y^\tau_h = r_h(x^\tau_h, a^\tau_h) + V^t_{m, h+1}(x^\tau_{h+1})$ denote the empirical value from specific transitions possessed by the agent, and $\lVert f \rVert$ denotes an appropriate regularization term based on the capacity of $f$ and $\cF$. To foster exploration, an additional bonus $\sigma^t_{m, h} : \cS \times \cA \rightarrow \bbR$ term is added that is inspired by the principle of optimism in the face of uncertainty, giving the final $Q$-value as,
\begin{equation}\label{eqn:q_ind}
 \resizebox{0.9\hsize}{!}{%
$Q^t_{m, h}(\cdot, \cdot) = \min\left\{ \left[\widehat Q^t_{m, h}+ \beta^t_{m, h}\sigma^t_{m, h}\right](\cdot, \cdot), H-h+1\right\},$%
}
\end{equation}
\begin{equation}\label{eqn:v_ind}
V^t_{m, h}(\cdot) = \max_{a \in \cA}Q^t_{m, h}(\cdot, a).
\end{equation}
Here $\beta^t_{m, h}$ is an appropriately chosen sequence. For any episode $t$, we denote $\bpi^t = \{\pi^t_m\}_{m \in \cM}$ as the (joint) greedy policy with respect to the $Q$-values $\{ Q^t_{m, h}\}_{h \in [H]}$ for each agent. While this describes the multiagent cooperative LSVI algorithm abstractly for any general function class $\cF$, we will now provide specific instantiations for each environment type.
\begin{algorithm}[t]
\caption{\textsc{Federated} \texttt{Coop-LSVI}}
\small
\label{alg:ind_homo}
\begin{algorithmic} %[1] enables line numbers
\STATE \textbf{Input}: $T, \Phi, H, \cF, K, S$, sequence $\beta_h = \{(\beta^t_{m, h})_{m, t}\}$.
\STATE \textbf{Initialize}: $\bS_1 = {\bf 0}, \bu_1 = {\bm 0}$.
\FOR{episode $t=1, 2, ..., T$}
\FOR{agent $m \in \cM$}
\STATE Receive initial state $x^t_{m, 1}$.
\STATE Set $V^t_{m, H+1}(\cdot) \leftarrow 0$.
\FOR{step $h = H, ..., 1$}
\STATE Compute $\bLambda^t_{m, h}$ using $\cU^t_{m, h}$ (Eqns.~\ref{eqn:y_ind_homo} and \ref{eqn:gram_ind_homo}).
\STATE Compute $\widehat Q^t_{m, h}$ and $\sigma^t_{m, h}$ (Eqns.~\ref{eqn:q_ind_homo} and ~\ref{eqn:s_ind_homo}).
\STATE Compute $Q^t_{m, h}(\cdot, \cdot)$ (Eqn.~\ref{eqn:q_ind})
\STATE Set $V^t_{m, h}(\cdot) \leftarrow \max_{a \in \cA}Q^t_{m, h}(\cdot, a)$.
\ENDFOR
\FOR{step $h=1, ..., H$}
\STATE Take action $a^t_{m, h} \leftarrow \argmax_{a \in \cA} Q^t_{m, h}(x^t_{m, h}, a)$.
\STATE Observe $r^t_{m, h}, x^t_{m, h+1}$.
\STATE $\cW^{t+1}_{m, h} \leftarrow \cW^t_{m, h} \cup (x^t_{m, h}, a^t_{m, h}, x^t_{m, h+1})$
\STATE Set $\bV^t_{m, h} \leftarrow \begin{bmatrix}
\bK^t_{m, h} & \bk^t_{m, h}(z^t_{m, h})^\top \\
\bk^t_{m, h}(z^t_{m, h}) & K(z^t_{m, h}, z^t_{m, h})
\end{bmatrix}$.
\IF{$\log\frac{\det\left(\bV^t_{m, h} + \lambda\bI\right)}{ \det\left(\bK^t_{m, h}+ \lambda\bI\right)} > \frac{S}{\Delta t_{m, h}}$}
\STATE \textsc{Synchronize}$(h) \leftarrow $ \textsc{True}.
\ENDIF
\ENDFOR
\ENDFOR
\IF{\textsc{Synchronize}}
\STATE [$\forall$ \textsc{Agents}] Set $\bar V^t_{H+1} = 0$
\FOR{step $h = H, ..., 1$}
\STATE [$\forall$ \textsc{Agents}] Compute $\y^t_{m, h}$ (Eqn.~\ref{eqn:ind_homo_delta_q}).
\STATE [$\forall$ \textsc{Agents}] Send $\delta\bLambda^t_{m, h}, \delta\y^t_{m, h} \rightarrow$ \textsc{Server}.
\STATE [\textsc{Server}] Aggregate $\delta\bLambda^t_{h} \leftarrow \sum_{m \in \cM} \delta\bLambda^t_{m, h}$.
\STATE [\textsc{Server}] Aggregate $\y^t_{h} \leftarrow \sum_{m \in \cM} \y^t_{m, h}$.
\STATE [\textsc{Server}] Communicate $\delta\bLambda^t_{h}, \y^t_{h}$ to each agent.
\STATE [$\forall$ \textsc{Agents}] Set $\bLambda^t_{m, h} \leftarrow \bLambda^t_{m, h} + \delta\bLambda^t_{h}$.
\STATE [$\forall$ \textsc{Agents}] Compute $\w^t_{m, h}$ (Eqn.~\ref{eqn:w_homo_ind}).
\STATE [$\forall$ \textsc{Agents}] Compute $\bar V^t_{h}$ (Eqn.~\ref{eqn:v_ind}).
\STATE [$\forall$ \textsc{Agents}] Set $\delta\bLambda^t_{m, h} \leftarrow {\bm 0}, \Delta t_{m, h} \leftarrow 0$. 
\ENDFOR
\ENDIF
\ENDFOR
\end{algorithmic}
\end{algorithm}
\textbf{Warm-Up: Homogenous MDPs.} In the homogenous setting, the transition functions $\bbP_{m, h}$ and reward functions $r_{m, h}$ are identical for all agents and can be given by $\bbP_h$ and $r_h$ respectively for any episode $h \in [H]$. This environment corresponds to distributed applications, e.g., federated and concurrent reinforcement learning. We assume here that $\cF$ is an RKHS $\cH$ with kernel $K$, and the penalty $\lVert f \rVert$ is the ridge penalty in $\cH$. Furthermore, we fix a threshold constant $S$ that determines the amount of communication between the agents. The algorithm is summarized in Algorithm~\ref{alg:ind_homo}.

In a nutshell, the algorithm operates by each agent executing a local kernelised LSVI and then synchronizing observations between other agents if a particular threshold condition is met every episode. Specifically, for each $t \in [T]$, each agent $m \in \cM$ obtains a sequence of value functions $\{Q^t_{m, h}\}_{h \in [H]}$ by iteratively performing kernel ridge regressions from the \textit{multi-agent} history available from the previous $t-1$ episodes. Assume that for any step $h$, the previous synchronization round occured after episode $t_{s, h}$. Then, the set of transitions available to agent $m \in \cM$ for any step $h$ before episode $t$ can be given by,
\begin{multline*}
\cU^t_{m, h} = \left\{ \cup \left( x^\tau_{n, h}, a^\tau_{n, h}, x^\tau_{n, h+1}\right)_{n \in \cM, \tau \in [t_{s, h}]}\right\} \\
\bigcup \left\{ \cup \left( x^\tau_{m, h}, a^\tau_{m, h}, x^\tau_{m, h+1}\right)_{\tau=t_{s, h}+1}^{t-1}\right\}.
\end{multline*}
Then, each agent $m$ first sets $Q_{m, H+1}^t$ to be a zero function, and for any $h \in [H]$, solves the regression problem:
\begin{equation}
 \resizebox{0.9\hsize}{!}{%
$\widehat Q^t_{m, h} \leftarrow \underset{f \in \cF}{\argmin}\left\{\underset{(x, a, x') \in \cU^t_{m, h}}{\sum} \left[y_{m, h}- f(x, a)\right]^2 + \lambda\cdot\lVert f \rVert^2_\cH\right\}.$%
}
\end{equation}
Here, $\lambda > 0$ is a regularizer and the targets are
\begin{equation}\label{eqn:y_ind_homo}
    y_{m, h}(x, a, x') = r_h(x, a) + V^t_{m, h+1}(x')
\end{equation}
Subsequently, $Q^t_{m, h}$ and $V^t_{m, h}$ are obtained using Equations~\ref{eqn:q_ind} and~\ref{eqn:v_ind}. Let $\sigma_\tau$ be an ordering of $\cU^t_{m, h}$ of length $U^t_{m, h}$. Then, we denote the target vector $\y^t_{m ,h} = [y_{m, h}(x_\tau, a_\tau, a'_\tau)]_{\tau \in \sigma_\tau}$. Furthermore, recall the shortcut $z = (x, a)$ and let $\cZ = \cS \times \cA$, we can define the Gram matrix $\bK^t_{m, h} \in \bbR^{U^t_{m, h} \times U^t_{m, h}}$ and vector function $\bk^t_{m, h} : \cZ \rightarrow \bbR^{U^t_{m, h}}$ as,
\begin{equation}\label{eqn:gram_ind_homo}
 \resizebox{0.9\hsize}{!}{%
$\bK^t_{m, h} = [K(z, z')]_{z, z' \in \cU^t_{m, h}}, \bk^t_{m,h}(z) = [K(z, z')]_{z' \in \cU^t_{m, h}}.$%
}
\end{equation}
Then, we have that for any $z \in \cZ$,
\begin{equation}\label{eqn:q_ind_homo}
\widehat Q^t_{m, h}(z) = \bk^t_{m, h}(z)^\top\left(\bK^t_{m, h} + \lambda\bI\right)^{-1}\y^t_{m, h}.
\end{equation}
And correspondingly, the UCB bonus is given as,
\begin{equation}\label{eqn:s_ind_homo}
 \resizebox{0.9\hsize}{!}{%
$\sigma^t_{m, h}(z)^2 = \lambda^{-1}\left[K(z, z) - \bk^t_{m, h}(z)^\top\left(\bK^t_{m, h} + \lambda\bI\right)^{-1}\bk^t_{m, h}(z)\right].$%
}
\end{equation}
This exploration bonus is similar to that of Gaussian process (GP) optimization~\citep{srinivas2009gaussian} and linear bandit~\citep{abbasi2011improved} algorithms, and it can be interpreted as the posterior variance of a Gaussian process regression. The motivation for adding the UCB term is similar to that in the bandit and GP case, to adequately overestimate the uncertainty in the ridge regression solution. When $\beta^t_{m, h}$ is appropriately selected, the $Q-$values are such that $Q^t_{m, h} \geq \bbT^\star_{m, h}Q^t_{m, h+1} = Q^\star_{m, h}$ with high probability, which is the foundation to bounding the regret.

After computing $Q-$values, each agent interacts with their MDP by executing the greedy policy with respect to the $Q-$values for each step $h \in [H]$. After each step, if any agent's personal Gram matrix for step $h$ satisfies the determinant condition with threshold $S$ (step~\ref{step:alg_ind_homo} of Algorithm~\ref{alg:ind_homo}), then it signals a synchronization with the server upon which the agents synchronize observations via the server. We can demonstrate the complexity of communication as a function of $S$.
\begin{proposition}[Communication Complexity]
\label{prop:communication_complexity}
tIf Algorithm~\ref{alg:ind_homo} is run with threshold $S$, then the total number of episodes with communication is upper bounded by $ 2H\sqrt{(T/S)\cdot\Gamma(MT)}+4H$.
\end{proposition}
The above result demonstrates that when $S = o(T)$, it is possible to ensure that the agents communicate only in a constant number of episodes. To present guarantees on the regret incurred by the algorithm, we first provide a few necessary assumptions on the environment.
\begin{assumption}[Complexity Bound for Bellman operators]
Let $R_Q > 0$ be a constant, and define the RKHS ball $\cQ^\star = \left\{ f \in \cH : \lVert f \rVert_\cH \leq R_Q\right\}$. It is assumed that $\forall \ h \in [H], m \in \cM$ and any $Q: \cS \times \cA \rightarrow [0, H]$, the Bellman operator $\bbT^\star_{m, h}$ projects $Q$ into the ball $\cQ^\star$, i.e., $\bbT^\star_{m, h}Q \in \cQ^\star$.
\label{assumption:bellman_scalar}
\end{assumption}
\begin{assumption}[Eigenvalue decay]
In the multi-agent independent environment, the Kernel integral operator defined over $\cL^2(\cZ)$ has countable and positive eigenvalues $\{\sigma_i\}_{i \geq 1}$ and corresponding eigenfunctions $\{\psi_i\}_{i \geq 1}$ that form an orthonormal basis of $\cL^2(\cZ)$ (by Mercer's Theorem~\citep{mercer1909xvi}). We assume that  $\sup_{z \in \cZ} K(z,z) \leq 1$ and the eigenvalues $\{\sigma_i\}_{i \geq 1}$ decay $\gamma-$exponentially for some $\gamma > 0$, i.e., for some absolute constants $C_1$ and $C_2$ such that $\sigma_j \leq C_1\cdot\exp\left(-C_2\cdot j^\gamma\right)$ for all $j \geq 1$. We additionally assume that there exists $\tau \in (0, 0.5)$ and a constant $C_\psi > 0$ such that $\sup_{z \in \cZ} \sigma^\tau_j\cdot|\psi_j(z)| \leq C_\psi \ \forall \ j \geq 1$.
\label{assumption:eigenvalue_scalar}
\end{assumption}
Assumption~\ref{assumption:bellman_scalar} ensures that $\cQ^\star$ contains the optimal value functions, and ensures no additional approximation bias when estimating $Q^\star_{m, h}$, and is identical to assumptions made in the statistical RL literature~\citep{}. Assumption~\ref{assumption:eigenvalue_scalar} is made to simplify the effective dimension of the kernel $K$, and is satisfied by commonly used kernels, e.g., squared-exponential, which satisfies the assumption with $\gamma = 1/d$. See~\citep{} for more details on such eigenvalue assumptions. We now present the main results for the homogenous setting.
\begin{theorem}
\label{thm:ind_homo}
Algorithm~\ref{alg:ind_homo} when run on $M$ agents with communication threshold $S$, $\beta_t = \cO(H\sqrt{\log tMH})$ and $\lambda = 1 - (MTH)^{-1}$ obtains the following cumulative regret after $T$ episodes, with probability at least $1-\alpha$,
\begin{equation*} 
\resizebox{0.9\hsize}{!}{%
$\regret(T)=\widetilde\cO\left(H^2\left(M\sqrt{S} + \sqrt{MT}\right)\sqrt{\log\left(\frac{1}{\alpha}\right)}\right).$%
}
\end{equation*}
\end{theorem}
Theorem~\ref{thm:ind_homo} suggests that the appropriate scaling of the parameters $\beta$ and $\lambda$ can ensure sublinear group regret. Similar to the analysis present in the single-agent linear~\citep{jin2020provably} and kernel~\citep{yang2020provably} function approximation settings, our analysis admits a dependence on the function class $\cH$ via the $\ell_\infty-$covering number and the effective dimension, which we simplify in Theorem~\ref{thm:ind_homo} by selecting appropriate values of the parameters. In its general form, the regret scales as $\cO\left(H^2\left(M\sqrt{S} + \sqrt{MT\log\cN_\infty(\epsilon^\star)}\right)\sqrt{\log\left(\frac{1}{\alpha}\right)}\right)$, where $\cN_\infty(\epsilon)$ is the $\epsilon$-covering number of $\cH$ under the $\ell_\infty$ norm, and $\epsilon^\star = \cO(H\cdot\Gamma(MT)/T)$, where $\Gamma$ denotes the information gain as in Definition~\ref{def:infogain_homo}. We elaborate on this connection in more detail in the full proof. 

The aspect central to the multi-agent analysis is the dependence on the communication threshold parameter $S$. If the agents communicate every round, i.e., $S = \cO(1)$, then we observe that the cumulative regret is $\widetilde\cO(\sqrt{MT})$, matching the centralized setting. With no communication, the agents simply operate independently and the regret incurred is $\widetilde\cO(M\sqrt{T})$, matching the group regret incurred by $M$ isolated agents. Furthermore, with $S = \cO(T\cdot\Gamma(MT)/M^2)$ we observe that with a total of $\cO(HM^3)$ episodes with communication, we recover a group regret of $\widetilde\cO(\sqrt{MT})$.

The above algorithm assumes that the underlying MDPs each agent interacts with are identical. We now present an extension of this algorithm that generalizes to the case when the underlying MDPs are different. In order to effectively transfer knowledge from a different agents' MDP, we require that both the transition function $\bbP$ and the reward function be ``close'' to each other. We formalize this via the Bellman optimality operators. 

\begin{assumption}
\label{assumption:bellman_hetero}
In the heterogenous setting, we assume that the heterogeneity within the Bellman optimality operators is small, i.e. for some constant $R_I \ll R_Q$,
\begin{align*}
    \sup_{Q : \cZ \rightarrow [0, H], h \in [H]} \sum_{i, j}^M \left\lVert (\bbT^\star_{i, h} - \bbT^\star_{j, h})(Q) \right\rVert_\cH \leq \sqrt{M}R_I.
\end{align*}
\end{assumption}
Assumption~\ref{assumption:bellman_hetero} encapsulates the notion of similarity between two MDPs, where we essentially require the optimal Bellman operators at each step $h$ to be ``close'' in the function space $\cH$ compared to their individual norms in $\cH$. For example, when $\cH$ is linear, this translates to an $\ell_2$ constraint between the projected (linear) $Q$ functions. This assumption is essentially an extension of the heterogeneity constraints in the multi-agent contextual bandit literature~\citep{cesa2013gang, li2016collaborative} to MDPs. Additionally, Assumption~\ref{assumption:bellman_hetero} does not directly impose any constraints on the optimal policy itself for any agent.

Our algorithm for the heterogenous setting is different from the homogenous case, where the goal was to only balance communication with the estimation error. Here, each agent essentially leverages the similarity between the transition functions to create stronger estimators for the Bellman operator $\bbT^\star$ at each step, via Assumption~\ref{assumption:bellman_hetero}. Consider the matrix $\bL \in \bbR^{M \times M}$ given by,
\begin{align}
    \bL &= \frac{1}{M}\left((M+1)\bI_M - {\mathbf 1}_M{\mathbf 1}_M^\top\right).
\end{align}
The matrix $\bL$ can be thought of as a (renormalized) Laplacian of a complete graph with $M$ vertices. The goal of the algorithm is for each agent to \textit{simultaneously} estimate the value functions for \textit{all agents} with the observations available to them, by constructing a function whose norm is controlled in terms of $R_I$ and $R_Q$. We achieve this by learning a function over the product space $\cZ \times \cM$ (where $\cM = [M]$). Consider the following features\footnote{$\otimes$ refers to the Kronecker product.}:
\begin{align}
    \bomega(l, x, a) &= \left[\underbrace{{\bm 0}_\cH, ...}_{(l-1)\text{ times}}, \bphi(x, a)^\top, \underbrace{ ..., {\bm 0}_\cH}_{(M-l)\text{ times}} \right]^\top, \\
    \btphi(l, x, a) &= \bA^{- 1/2}\bomega(l, x, a), \text{ where, } \bA = \bL \otimes \bI_\cH.
\end{align}
Here $\cH$ is the function class (ref. Assumption~\ref{assumption:bellman_scalar}) and $\bphi$ is its corresponding feature. We denote the RKHS corresponding to the augmented feature $\btphi$ as $\ctH$ and the corresponding kernel as $\widetilde K = \btphi^\top\btphi$. For any agent $m \in M$, let the estimated value function for some other agent $n$ at episode $t$ and step $h$ be given by $V^t_{m \rightarrow n, h}$. Then, in contrast to the homogenous case, here the agent solves the \textit{heterogenous} value iteration problem, given by:
\begin{equation}\label{eqn:ind_hetero_main}
 \resizebox{0.9\hsize}{!}{%
    $f^t_{m, h} = \underset{f \in \ctH}{\argmin} \underset{ \cU^t_{s, h}}{\sum} \left[ y^t_{m, h}(l, x, a, x') - f(l, x, a) \right]^2 + \lambda \lVert f \rVert_{\ctH}^2.$
    }
\end{equation}
Where $y^t_{m, h}(l, x, a, x') = r_{l, h}(x, a) + V^t_{m \rightarrow l, h+1}(x')$ are the targets for the regression, and $V^t_{m \rightarrow n, H+1} = 0$ for all $m, n \in \cM$ as in the homogenous case. After obtaining $f^t_{m, h}$ (which is defined over $\cZ \times \cH$), each agent $m \in \cM$ estimates the $Q-$functions $\widehat Q^t_{m \rightarrow n, h} = f^t_{m, h}(\cdot, n)$ and value functions $V^t_{m \rightarrow n, h}(x) = \max_{a \in \cA} \widehat Q^t_{m \rightarrow n, h}(x, a)$ for all agents $n \in \cM$. Similar to the homogenous case, the policy is a greedy policy with respct to a UCB of the estimated $Q-$values. However, in this case, the UCB is calculated using the confidence interval of $f^t_{m, h}$ (and not just the $Q-$values). The intuition for this is that because Assumption~\ref{assumption:bellman_hetero} guarantees that the MDPs of different agents are ``close'', $f^t_{m, h}$ will have a small confidence interval as well. Now, to describe the solution to Equation~\ref{eqn:ind_hetero_main} and the relevant confidence interval we introduce some additional notation.Let $\sigma_\tau$ be an ordering of $\cU^t_{m, h}$ of length $U^t_{m, h}$. Then, we denote the target vector $\y^t_{m ,h} = [y_{m, h}(l_\tau, x_\tau, a_\tau, a'_\tau)]_{\tau \in \sigma_\tau}$. Furthermore, consider the shortcut $\tilde z = (l, x, a)$ and let $\ctZ = \cZ \times [M]$, we can define the Gram matrix $\btK^t_{m, h} \in \bbR^{U^t_{m, h} \times U^t_{m, h}}$ and vector function $\btk^t_{m, h} : \ctZ \rightarrow \bbR^{U^t_{m, h}}$ as,
\begin{equation}\label{eqn:gram_ind_hetero}
 \resizebox{0.8\hsize}{!}{%
$\btK^t_{m, h} = [\tilde K(z, z')]_{z, z' \in \cU^t_{m, h}}, \btk^t_{m,h}(z) = [\tilde K(z, z')]_{z' \in \cU^t_{m, h}}.$%
}
\end{equation}
Then, we have that $f^t_{m, h}$ can be given as, for any $\tilde z \in \ctZ$,
\begin{equation}
    f^t_{m, h}(\tilde z) = \btk^t_{m, h}(\tilde z)^\top\left(\btK^t_{m, h} + \lambda\bI\right)^{-1}\y^t_{m, h}
\end{equation}
Using this, we set the $Q-$value as, for any $z \in \cZ$,
\begin{equation}\label{eqn:q_ind_hetero}
\widehat Q^t_{m, h}(z) =f^t_{m, h}(z, m).
\end{equation}
In contrast to the homogenous case, the confidence bonus is given by 
\begin{equation}
 \resizebox{0.9\hsize}{!}{%
$\sigma^t_{m, h}(z)^2 = \lambda^{-1}\left[K(z, z) - \bk^t_{m, h}(z)^\top\left(\bK^t_{m, h} + \lambda\bI\right)^{-1}\bk^t_{m, h}(z)\right].$%
}
\end{equation}
\begin{equation}
    ss
\end{equation}
\section{Algorithm for Markov Games}

